P4: Towards private, personalized, and Peer-to-Peer learning

Personalized learning is a proposed approach to address the problem of data heterogeneity in collaborative machine learning. In a decentralized setting, the two main challenges of personalization are client clustering and data privacy. In this paper, we address these challenges by developing P4 (Personalized Private Peer-to-Peer) a method that ensures that each client receives a personalized model while maintaining differential privacy guarantee of each client's local dataset during and after the training. Our approach includes the design of a lightweight algorithm to identify similar clients and group them in a private, peer-to-peer (P2P) manner. Once grouped, we develop differentially-private knowledge distillation for clients to co-train with minimal impact on accuracy. We evaluate our proposed method on three benchmark datasets (FEMNIST or Federated EMNIST, CIFAR-10 and CIFAR-100) and two different neural network architectures (Linear and CNN-based networks) across a range of privacy parameters. The results demonstrate the potential of P4, as it outperforms the state-of-the-art of differential private P2P by up to 40 percent in terms of accuracy. We also show the practicality of P4 by implementing it on resource constrained devices, and validating that it has minimal overhead, e.g., about 7 seconds to run collaborative training between two clients.

==> paper/MacrosMarkup.tex <==
% For TeXshop: make it LaTeX the root file if you cmt-T here.
% !TEX root = main.tex

%%% Macros for "in progress" artefacts: colours, funny footnotes, funny endnotes, showing labels etc.
%%% MacrosMarkup Carroll Morgan 21 September 2018 and Kostas Chatzikokolakis.
\providecommand{\UsePackageFor}[2]{ \ifx#2\undefined\usepackage{#1}\fi }

\UsePackageFor{amssymb}{\boxtimes}
\usepackage[normalem]{ulem}		% For strikethroughs.
\usepackage{bbding}				% For the small pencil.
%\usepackage{dingbat}			% For pointing hand.
\usepackage{endnotes}			% For endnotes.
\usepackage{hyperref}			% For hyperlinks to and from endnotes.
\usepackage{hyperendnotes}	% Make \ref's to endnotes work correctly with hyperref.
\usepackage{pdfcolfoot}			% Fixes issues with coloured footnotes that break across pages.

% pdfcolfoot tries to restore footnote colours that break across pages, which might cause
% a colour to escape to the next footnote. So we use our own wrapper of \footnote,\footnotetext
% and enclose the footnote in a dummy FootnoteContent environment, so that the colour is restored.
% (Note: MacrosLabels applies the exact same patch for a different purpose.)
%
\ifdefined\OrigFootnote\relax\else% might be already applied by MacrosLabels
	\newenvironment{FootnoteContent}{}{}
	\let\OrigFootnote\footnote
	\let\OrigFootnoteText\footnotetext
	\renewcommand{\footnotetext}[1]{\OrigFootnoteText{\begin{FootnoteContent}#1\end{FootnoteContent}}}
	\renewcommand{\footnote    }[1]{\OrigFootnote    {\begin{FootnoteContent}#1\end{FootnoteContent}}}
\fi

%%% Colours and markups
%
\definecolor{PurplePlum}{rgb}{0.1,0,0.55} 
\definecolor{Brown}{rgb}{0.5,.25,0}
\definecolor{Orange}{rgb}{1,.3,0}
\definecolor{Gray}{rgb}{.7,.7,.7}
\definecolor{DarkGreen}{rgb}{.1,.41,.1}
%\definecolor{Black}{rgb}{0,0,0}
%\definecolor{PineGreen}{rgb}{0,0.5,0.5}
%\definecolor{Green}{rgb}{0,.5,0}

\newif\ifBleck
\newcommand\Bleck {\Blecktrue} % Carry out all deletes and replacements; remove all footnotes/endnotes; make everything black.

% To check that all colouring-calls to markup functions have been removed, disable \Bleck and enable Colour->\undef.
\newcommand\Colour[1] {\color{#1}}
%\renewcommand\Colour[1] {\undef} % Enable this to check that no colours are used by Markups.

\newcommand\PrintToCLinks{	% This prints the actual links.
  {\Colour{blue}\mbox{
    \hyperlink{w1619}{\sf$\rightarrow$~top}\quad
    \hyperlink{w1031}{\sf$\rightarrow$~toc}\quad
    \hyperlink{w1148}{\sf$\rightarrow$~lof}\quad
    \hyperlink{GreenRoom}{\sf$\rightarrow$~gr}\quad
    \hyperlink{EndNotes}{\sf$\rightarrow$~en}\quad
    \hyperlink{Sargasso}{\sf$\rightarrow$~sg}\quad
    \hyperlink{Index}{\sf$\rightarrow$~idx}
  }}
}
% http://tex.stackexchange.com/questions/201348/why-doesnt-makeatletter-work-inside-newcommand
\makeatletter % must be outside \newcommand
\newcommand\ToCLinks{
  % create "top" target
  \ifx\@onlypreamble\@notprerr		% If in document...
    \hypertarget{w1619}{}			% ...do it now.
  \else
    \AtBeginDocument{\hypertarget{w1619}{}}	% But in the preamble, delay.
  \fi

  \ifBleck\else	% 1031: Put hyperlink to ToC  and GR at bottom of every page.
    			% KOMA has \cofoot and \cefoot commands for adding a centered footer that
    			% co-exists with the page's normal footer. If available we use them.
    \ifdefined\cofoot
      \cofoot{\PrintToCLinks}
      \cefoot{\PrintToCLinks}
    \else
      \def\@oddfoot{\PrintToCLinks}
      \def\@evenfoot{\PrintToCLinks}
    \fi
 \fi
}
\makeatother

\newif\ifEndNotes % 0831: Workaround for endnotes-bug: missing ".ent" file when there are no endnotes.

\newcommand\FnSym{{\scriptsize\PencilLeftDown\kern.1em}}		% Needs bbding.
\newcommand\EnSym {{$\bigtriangledown$}}
\newcommand\Fn[1] {[\FnSym\ref{#1}]}						% For referring to footnotes.
\newcommand\En[1] {[\EnSym\ref{#1}]}						% For referring to EndNotes.
\newcommand\ENSection[1] {\par\noindent\textbf{\large #1}\par\medskip}
\newcommand\ENSubsection[1] {\par\noindent\textbf{#1}\par\medskip}
\newcommand\ENItem[1] {\item[\textbf{#1}]~\par}
%\newcommand\NA[1] {{\Colour{#1}\large\phone}~}

%%%  \MakeMarkups[optionalComment]{prefixLetter}{textModifier}
%%%  One for each person: for example C for prefixLetter and \Colour{blue} for textModifier would be
%%%
%%%     \MakeMarkups[optionalComment]{C}{\Colour{blue}}
%%%
%%%  A possible use for optionalComment is to give the person's name.
%%%
%%%  "Disabling" a markup (or all of them) makes the document look as if that (those) markups had
%%%  been carried out. Replacements/deletions are done; footnotes, endnotes and t-comments are
%%%  removed; the document becomes black.
%%%
%%%  Disable all markups with macro \Bleck; also Green Room, Sargasso and Endnotes are suppressed.
%%%  Disable individual markup (rather than all via \Bleck) by eg \MakeMarkups[0]{C}{...}
%%%  Re-enable individual markups in spite of \Bleck with \MakeMarkups[1]{C}{...}
%%%
%%%  A help "how-to" can be printed any time after calling \MakeMarkups by \MarkupsHowto.
%%%  The "how-to" can be made shorter (just list the markups, no help) by \MarkupsHowtoPrintedtrue.
%%%

% Very sneaky!
\def\MarkupsHowto{} % How-to content, we add in every \MakeMarkups, use \MarkupHowto to print.
\newcommand{\MarkupsHowtoAdd}[1]{\expandafter\def\expandafter\MarkupsHowto\expandafter{\MarkupsHowto{}#1}} % adds to \MarkupsHowto

\newif\ifMarkupsHowtoPrinted %1121: Print help text only once. (Note: this is actually set to true when the how-to is _printed_.)
\newcommand\MakeMarkupsCalledtrue {\MarkupsHowtoPrintedtrue} % Temporary.
\newif\ifSuppress % Used to decide whether to suppress individual markups.

%%% Call this once for every markup'er you want to have.
\newcommand\MakeMarkups[3][.]{%1119

    % Suppress these markups if (Bleck OR [0]) and not [1].
     \Suppressfalse
     \ifBleck\Suppresstrue\fi
     \ifx0#1\Suppresstrue\fi
     \ifx1#1\Suppressfalse\fi
     
    % \Xx: Change to colour.
     \expandafter\providecommand\csname#2x\endcsname {} % 1613: Using providecommand this way allows MakeMarkups to be called more than once for a particular person.
     \ifSuppress\expandafter\renewcommand\csname#2x\endcsname{\relax}\else
                       \expandafter\renewcommand\csname#2x\endcsname{#3}\fi
                       
    % \X{#1}: Put #1 in colour.
     \expandafter\providecommand\csname#2\endcsname {} % 1613.
     \ifSuppress\expandafter\renewcommand\csname#2\endcsname[1]{##1}\else
                       \expandafter\renewcommand\csname#2\endcsname[1]{{\csname#2x\endcsname##1}}\fi

    % \Xd{#1}: Delete (strikeout) #1; needs ulem package.
     \expandafter\providecommand\csname#2d\endcsname {} % 1613.
     \ifSuppress\expandafter\renewcommand\csname#2d\endcsname[1]{\relax}\else
                       \expandafter\renewcommand\csname#2d\endcsname[1]{{\csname#2x\endcsname\sout{##1}}}\fi
                       
   % \Xr{#1}{#2}: Replace #1 with #2.
     \expandafter\providecommand\csname#2r\endcsname {} % 1613.
     \ifSuppress\expandafter\renewcommand\csname#2r\endcsname[2]{{##2}}\else
                       \expandafter\renewcommand\csname#2r\endcsname[2]{\csname#2d\endcsname{##1} \csname#2\endcsname{##2}}\fi

   % \Xi{#1}: Insert #1.
     \expandafter\providecommand\csname#2i\endcsname {} % 1613.
     \ifSuppress\expandafter\renewcommand\csname#2i\endcsname[1]{\relax}\else
                       \expandafter\renewcommand\csname#2i\endcsname[1]{\csname#2\endcsname{##1}}\fi

    % \Xt{#1}: Like \Xd{#1} but without strikeout; use where \Xf{#1} not allowed because e.g. "not in outer par mode".
     \expandafter\providecommand\csname#2t\endcsname {} % 1613.
     \ifSuppress\expandafter\renewcommand\csname#2t\endcsname[1]{\relax}\else
                       \expandafter\renewcommand\csname#2t\endcsname[1]{{\csname#2x\endcsname{\mbox{$\langle\!\langle$}##1{\csname#2x\endcsname\mbox{$\rangle\!\rangle$}}}}}\fi 

    % \Xb[#1]: Put bookmark in the margin, with optional parameter.
     \expandafter\providecommand\csname#2b\endcsname {} % 1613.
     \ifSuppress\expandafter\renewcommand\csname#2b\endcsname[1][empty]{\relax}\else 
                       \expandafter\renewcommand\csname#2b\endcsname[1][\empty]{\ifx\empty##1\empty
                       	\label{#2-bookmark} % With hyperlinks you can jump directly to your bookmark by clicking on an appropriate \pageref.
                              \marginpar [\raggedleft\csname#2\endcsname{{\footnotesize\fbox{#2 working here}}~$\Longrightarrow$}]
                                                {\csname#2\endcsname{$\Longleftarrow$~{\footnotesize\fbox{#2 working here}}}}
                       \else % No label if there's an explicit parameter.
                       	  % In general \ifx\empty#1\empty succeeds if the argument #1 is empty, or begins with \empty:
    			  % in the first case \if gets true for \empty=\empty;
    			  % in the second case it gets true for \empty=\empty (in #1), and possibly sticks in the rest of #1.
    			  % Anything else gives false.
                       	\marginpar [\raggedleft\csname#2\endcsname{\ifx\empty##1\empty\else\fbox{\tiny\parbox{8em}{\raggedright##1}}~\fi$\Longrightarrow$}]
                                                {\csname#2\endcsname{$\Longleftarrow$\ifx\empty##1\empty\else~{\tiny\fbox{\parbox{8em}{\raggedright##1}}}\fi}}\fi}\fi

    % \XTD: This person to do.
     \expandafter\providecommand\csname#2TD\endcsname {} % 1613.
     \ifSuppress\expandafter\renewcommand\csname#2TD\endcsname{\relax}\else
                       \expandafter\renewcommand\csname#2TD\endcsname{\csname#2\endcsname{\fbox{#2 to do}}}\fi

    % \XBar: Left by other people: delete when you're happy.
     \expandafter\providecommand\csname#2Bar\endcsname {} % 1613.
     \ifSuppress\expandafter\renewcommand\csname#2Bar\endcsname{\relax}\else
                       \expandafter\renewcommand\csname#2Bar\endcsname{\csname#2\endcsname{\scriptsize\XSolidBrush}}\fi

    % \Xf{#1}: Make coloured "footnote #1 to self".
     \expandafter\providecommand\csname#2f\endcsname {} % 1613.
     \ifSuppress\expandafter\renewcommand\csname#2f\endcsname[2][]{\relax}\else
      \expandafter\renewcommand\csname#2f\endcsname[2][\empty]{ % Have forgotten what the optional parameter was for.
        {\mbox{\csname#2x\endcsname\tiny$\boxtimes$}\marginpar{\hsize1cm\csname#2x\endcsname\fbox{\FnSym\footnotemark}}\relax 
        \footnotetext{\csname#2x\endcsname##2}}}\fi

    % \Xe{#1}: An endnote: like \Xf, but longer text #1 put at the end of the document.
     \expandafter\providecommand\csname#2e\endcsname {}% 1613.
     \ifSuppress\expandafter\renewcommand\csname#2e\endcsname[1]{\relax}\else%
      \expandafter\renewcommand\csname#2e\endcsname[1]{%
       \global\EndNotestrue%0831
       \mbox{\scriptsize\csname#2x\endcsname$\boxtimes$}\relax%
       \marginpar{\hsize1cm\csname#2x\endcsname\fbox{\EnSym\endnotemark%
                          \hypertarget{ENmark\thepage-\theendnote}{}~\hyperlink{ENtext\thepage-\theendnote}{{\Colour{blue}$\downarrow$}}}%
       }%
       {% 1641 Make \z,\zz local.
        \def\zz{\noexpand#3}%
%     \edef\z{~{\zz[Endnote \theendnote\ % Can't get this to work when #3 is several tokens. CCM 180521.
        \edef\z{~{[Endnote \theendnote\ %
        on p.\noexpand\hypertarget{ENtext\thepage-\theendnote}{}\thepage%
                    ~\noexpand\hyperlink{ENmark\thepage-\theendnote}{{\noexpand\Colour{blue}$\uparrow$}}]}%
        }%
        \expandafter\endnotetext\expandafter{\z\vspace{2ex}\\ ##1\newpage}%
       }%1641
      }\fi

    % \Xn{#1}: An endnote with no reference: like \Xe, but only a tiny marginal number is put in the text.
    % Useful in the final stages when you're removing notes (because they are distracting)
    % but still you might want to have a final look at the endnotes that were there
    % before you go for submission.
     \expandafter\providecommand\csname#2n\endcsname {}% 1613.
     \ifSuppress\expandafter\renewcommand\csname#2n\endcsname[1]{\relax}\else%
      \expandafter\renewcommand\csname#2n\endcsname[1]{%
       \global\EndNotestrue%0831
    %  \mbox{\scriptsize\csname#2x\endcsname$\boxtimes$}\relax
    %  \marginpar{\csname#2x\endcsname\fbox{\EnSym\endnotemark
    %                     \hypertarget{ENmark\thepage-\theendnote}{}~\hyperlink{ENtext\thepage-\theendnote}{{\Colour{blue}$\downarrow$}}}
    % }
    \marginpar{{\tiny\endnotemark}\hypertarget{ENmark\thepage-\theendnote}{}~\hyperlink{ENtext\thepage-\theendnote}{}}
       {% 1641 Make \z,\zz local.
        \def\zz{\noexpand#3}%
        \edef\z{~{\zz[Endnote (deferred) % \theendnote\ 
        from p.\noexpand\hypertarget{ENtext\thepage-\theendnote}{}\thepage%
    %\noexpand\hyperlink{ENmark\thepage-\theendnote}{{\noexpand\Colour{blue}$\uparrow$}}
        ]}%
        }%
        \expandafter\endnotetext\expandafter{\z\vspace{2ex}\\ ##1\newpage}%
       }%1641
      }\fi

    % Like \Xf and \Xe together --- Use \Xfe[<file name for endnote>]{Short footnote about file's contents.}
     \expandafter\providecommand\csname#2fe\endcsname {} % 1613.
     \ifSuppress\expandafter\renewcommand\csname#2fe\endcsname[2][]{\relax}\else %1538
      \expandafter\renewcommand\csname#2fe\endcsname[2][]{ % 1540: \File is local.
       \def\File{##1}\relax
       \ifx\File\empty\csname#2f\endcsname{##2}\else % 1536: Without file, behave like \Xf.
        \global\EndNotestrue %0831
        \mbox{\scriptsize\csname#2x\endcsname$\boxtimes$}
        \marginpar{\csname#2x\endcsname\fbox{\FnSym\footnotemark}}\relax
        \footnotetext{~\csname#2x\endcsname##2\
                             --- See [\EnSym\endnotemark\hypertarget{ENmark\thepage-\theendnote}{}
                             \kern-.2em\hyperlink{ENtext\thepage-\theendnote}{{\Colour{blue}$\downarrow$}}].}\relax
       { % 1641 Make \z,\zz local.
         \def\zz{\noexpand#3}
         \edef\z{~{\zz[Endnote~\thefootnote~on~p.\noexpand\hypertarget{ENtext\thepage-\theendnote}{}\thepage
                     ~\noexpand\hyperlink{ENmark\thepage-\theendnote}
                     {{\noexpand\Colour{blue}\kern-0.1em$\uparrow$}]}}
                     {\noexpand\footnotesize\noexpand\newline\noexpand\hspace*{2em} (~from file {\noexpand\tt\File.tex}~)}
         }    
         \expandafter\endnotetext\expandafter{\z~\par\input{##1}\newpage}
        } %1641
       \fi % 1536
      } % 1540
     \fi % 1538

    % "How-to" material printed by the first call to \MakeMarkups; suppress by \MarkupsHowtoPrintedtrue just before that first call.
    % Bleck removes the _whole footnote_ even if Suppress == false
     \ifSuppress\relax\else\ifBleck\relax\else%0749
      \MarkupsHowtoAdd{\par\csname#2t\endcsname{%1009
       $\backslash$\texttt{#2}$\cdots$\ markups are in \textbf{this} colour\ifx#1..\else\ifx1#1.\else, e.g.\ for #1.\fi\fi
       \ifMarkupsHowtoPrinted\relax\else %1121
        \global\MarkupsHowtoPrintedtrue %1121
        \begin{quote}\begin{tabular}{l@{\hspace{2em}}p{.7\linewidth}}
         \multicolumn{2}{l}{\texttt{$\backslash$MakeMarkups\ifx#1.\relax\else[#1]\fi\{#2\}\{{\it$\langle$colour command\/$\rangle$}\}}
         				 --- Defines the macros below:}\\
             & see comments at \texttt{$\backslash$MakeMarkups} definition. \\[1ex]
         \texttt{$\backslash$#2\{$\langle$text$\rangle$\}} & Sets \texttt{$\langle$text$\rangle$} in \texttt{#2}'s colour. \\
         \texttt{$\backslash$#2x} & Changes to \texttt{#2}'s colour (until end of context). \\
         \texttt{$\backslash$#2d\{$\langle$text$\rangle$\}} & Sets \texttt{$\langle$text$\rangle$} in \texttt{#2}'s colour with a strikethrough (i.e.\ delete). \\
         \texttt{$\backslash$#2r\{$\langle$this$\rangle$\}\{$\langle$that$\rangle$\}} &
          Strikes through \texttt{$\langle$this$\rangle$} and inserts \texttt{$\langle$that$\rangle$} (i.e.\ replace). \\
         \texttt{$\backslash$#2f\{$\langle$text$\rangle$\}} & Meta-comment: puts \texttt{$\langle$text$\rangle$} in a \texttt{#2}-footnote with a {\tiny$\boxtimes$} in the main text. \\
         \texttt{$\backslash$#2t\{$\langle$text$\rangle$\}} & Use for meta when  \texttt{$\backslash$#2f} isn't allowed (``Not in outer-par mode.'') \\
         \texttt{$\backslash$#2b[$\langle$optional$\rangle$]} & Marginal pointer, with label for hyper-linking directly there. \\
         \texttt{$\backslash$#2e\{$\langle$text$\rangle$\}} & Puts \texttt{$\langle$text$\rangle$} in a \texttt{#2}-endnote with a (big) $\boxtimes$ in the main text. \\[.5ex]
         \texttt{$\backslash$#2n\{$\langle$text$\rangle$\}} & Like \texttt{$\backslash$#2e}
         except there's no reference from the main text. Good for ``decluttering''
         when you still want to have the footnote- or endnote texts as reminders. \\[.5ex]
         \texttt{$\backslash$#2fe[$\langle$this$\rangle$]\{$\langle$that$\rangle$\}} & Makes a \texttt{$\backslash$#2f\{$\langle$that$\rangle$\}} that refers to a \\
           & \texttt{$\backslash$#2e\{$\langle$contents of file this.tex$\rangle$\}}. \\ 
           & Without the optional argument, acts as \texttt{$\backslash$#2f\{$\langle$that$\rangle$\}}. \\[.5ex]
         \texttt{$\backslash$#2Bar} & Inserts ``burn after reading'' symbol \csname#2Bar\endcsname, meaning
          \begin{quote}\begin{itemize}\setlength\itemsep{0pt}
           \item If yours is the only \csname#2Bar\endcsname\ in this (presumably someone else's) footnote, and you are happy that the footnote has been addressed,
           go ahead and comment-out the whole footnote. (The \csname#2Bar\endcsname\ is their request for you to ``approve and remove''.)
           \item If you are not happy, delete only your \csname#2Bar\endcsname\ and follow-on in the footnote
            (in your colour, i.e.\ with \texttt{$\backslash$#2x}) saying why you are not happy.
           \item If you are happy, but there are others' burn-after-reading symbols as well as yours, just delete yours; the other people have not yet responded.
          \end{itemize}
          \end{quote}
          The idea is that when everyone's happy, the last person will comment-out the meta-text. \\[0.5ex]
         \texttt{$\backslash$#2TD} & Inserts {\csname#2TD\endcsname}\ . \\
        \end{tabular}\end{quote}
       \fi
      }}%1009
     \fi\fi%0749
}%1119

\newcommand\Divider {~\vfill~\bigskip\hrule~\\\hrule~\bigskip} % For separating contributions in GreenRoom etc. Put in contributor's colour.

\newif\ifNoGreenRoom\newcommand\NoGreenRoom{\NoGreenRoomtrue}
\newcommand\MakeGreenRoom {\ifBleck\relax\else\ifNoGreenRoom\relax\else
% \cleardoublepage % Not necessary if \include'd.
% CCM Added "label-branding" 180524.
\newcommand\NewGRLabel[1] {\OldGRLabel{GreenRoom-##1}} % All Green-Room labels "branded".
 \newcommand\NewGRRef[1] % All Green-Room references take branded version if possible.
 {\expandafter\ifx\csname r@GreenRoom-##1\endcsname\relax\OldGRRef{##1}\else\OldGRRef{GreenRoom-##1}\fi}
 % Now swap them over.
 \let\OldGRLabel\label \let\label\NewGRLabel
 \let\OldGRRef\ref \let\ref\NewGRRef
 \hrule
 ~\\\begin{center}\Huge \hypertarget{GreenRoom}{Green Room}
 \end{center}~\\
 \hrule
\fi\fi}

\newcommand\EndGreenRoom  {\ifBleck\relax\else\ifNoGreenRoom\relax\else
% Swap them back.
\let\label\OldGRLabel
\let\ref\OldGRRef
\fi\fi}

\newif\ifNoEndNotes\newcommand\NoEndNotes{\NoEndNotestrue}
\newcommand\MakeEndNotes {\ifBleck\relax\else\ifNoEndNotes\relax\else
% \cleardoublepage % Not necessary if \include'd.
 \hrule\vspace{20pt}\begin{center}\ifEndNotes\Huge Endnotes\else\textit{No endnote macros were called in this run.}\fi\end{center}\vspace{20pt}\hrule
 {\parindent 0pt \parskip 2ex \def\enotesize{\normalsize} \def\notesname{} % Supress EndNotes title.
 \ifEndNotes\theendnotes\fi} %0831
\fi\fi}

\newif\ifNoSargasso\newcommand\NoSargasso{\NoSargassotrue}
\newcommand\MakeSargasso {
 % Localise labels and references to Sargasso itself, if possible.
 % Stuff In Sargasso might be a copy of earlier material, and we don't want the earlier labels to be overwritten.
 \hypertarget{Sargasso}{}
 \newcommand\NewLabel[1] {\OldLabel{Sargasso-##1}} % All Sargasso labels "branded".
 \newcommand\NewRef[1] % All Sargasso references take branded version if possible.
 {\expandafter\ifx\csname r@Sargasso-##1\endcsname\relax\OldRef{##1}\else\OldRef{Sargasso-##1}\fi}
 % Now swap them over.
 \let\OldLabel\label \let\label\NewLabel
 \let\OldRef\ref \let\ref\NewRef
 %
\ifBleck\end{document}\else\ifNoSargasso
\relax% \begin{center}\huge \textit{Sargasso suppressed in this run}\end{center}
\else
% \cleardoublepage % Not necessary if \include'd.
  \hrule
  ~\\\begin{center}\Huge Sargasso
  \end{center}~\\
  \hrule
 \fi\fi
}

\newcommand\EndSargasso  {\ifBleck\relax\else\ifNoSargasso\relax\else
% Swap them back.
\let\label\OldLabel
\let\ref\OldRef
\fi\fi}



\newcommand\EndDocument {\ifBleck\end{document}\fi} % Cut off the Green Room and the Sargasso when Bleck.

% For citations to be filled-in later: better than \cite{later} because \cite{later} generates undefined-reference warnings that might mask real ones.
% \Cite is -not- disabled by \Bleck, since \Bleck is supposed to make a version that is "OK to submit", and missing references is not "not OK".
% If necessary however (eg in a panic :-) you can enable \Bleck and disable \Cite, the latter by uncommenting the command following.
\newcommand\Cite[2][\empty] {{\Colour{red}\ifx#1\empty[#2]\else[#2,~#1]\fi}}
\newcommand\OpCit {[op.cit.]}
%\renewcommand\Cite[1] {\relax}

%%% End of \Markups


==> paper/parts/discussion.tex <==
Our work can be extended in a few ways. 
We used a similarity metric to group clients and conducted knowledge sharing within each group. 
We employed a simple approach to make groups based on limited sampling. 
Although this approach leads to good performance, optimizing the algorithm that makes groups based on sampled similarities could be a potential avenue for improvement. 
The optimization would be in terms of reducing communication overhead or grouping clients more precisely such that sampling has minor negative impact on the accuracy of the overall training algorithm. 
Additionally, we considered a setting with honest but curious clients. 
Improving \name to be robust against malicious clients that can share incorrect or harmful inputs that affect the training algorithm is another area for future work.

Moreover, the handcrafted feature is crucial in our design, enabling our algorithm to converge even with noisy gradients. The use of handcrafted features can be extended to other domains, such as text and audio, by employing techniques proposed in previous works \cite{manning1999foundations} and \cite{anden2014deep}, respectively.
